A Broadcast Authenticated Encryption with Keyword Search in the Standard Model: Tightly Secure in Multi-User, Multi-Challenge Settings

However, no known work considered the functionality requirement in its most realistic setting. We propose a new security definition of BAEKS in the multi-user (with adaptive corruptions) and multi-challenge (both in terms of ciphertext and trapdoor in an interleaved manner) settings. We also study the question of the unforgeability of BAEKS. In fact, our strong hiding requirement already implies a significant amount of unforgeability. We then propose a new BAEKS construction in the bilinear pairing groups. We prove this scheme achieves adaptive tight full-hiding security under (almost) standard MDDH assumptions. Restricting our BAEKS construction for a single receiver also gives an efficient and tightly secure PAEKS construction. We further run experiments to implement and evaluate our scheme.

==> Macro.tex <==
% \usepackage{titling}
% \newcommand{\subtitle}[1]{%
%   \posttitle{%
%     \par\end{center}
%     \begin{center}\LARGE#1\end{center}
%     \vskip0.5em}%
% }


\usepackage{stmaryrd}
\usepackage{etoolbox}
\usepackage{amsmath,amsthm} %Uncomment when not article
\allowdisplaybreaks
\usepackage{amssymb,amsbsy}
\usepackage{amsfonts}
% %\usepackage{mathtools}
% %\usepackage{marginnote}
% \usepackage{algorithm2e}
% \RestyleAlgo{boxed}
% %\usepackage{color,xcolor}
\usepackage{tcolorbox}
\usepackage{ifthen}
% \usepackage{color,xcolor}
\definecolor{darkblue}{rgb}{0,0,0.6}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{maroon}{rgb}{0.5,0.1,0.1}
\definecolor{dpurple}{rgb}{0.2,0,0.65}
\definecolor{darkviolet}{RGB}{130,95,141}
\definecolor{darkkhaki}{RGB}{189,183,107}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
\usepackage[%
%  dvipdfmx,  
 colorlinks=true,
 citecolor=darkspringgreen,
 linkcolor=ceruleanblue,
 urlcolor=ceruleanblue,
%  pagebackref=true,
 breaklinks=true
]{hyperref}
% \usepackage{hyperref}
\usepackage{cleveref}
% %\usepackage{latexsym}
% % \usepackage{almendra}
\usepackage[T1]{fontenc}
% \usepackage{lscape}
\usepackage{cases}
% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{remark}{\bf Remark}

\usepackage{mdframed}
\usepackage{booktabs}
\usepackage{algpseudocode}
\usepackage[lined,linesnumbered,commentsnumbered]{algorithm}
\usepackage[font=normalsize,format=plain,labelfont={up},labelsep=space,justification=centering]{caption}

\def\done{\color{green}done}
\def\notdone{\color{red}Noddun}

%\usepackage{newpxmath,newpxtext}

% new \oset macro:
\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-2\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother
\let\Bot\relax

% new bslash macro
\newcommand{\bslash}{\mathbin{
  \mathchoice{/\mkern-6mu/}% \displaystyle
    {/\mkern-6mu/}% \textstyle
    {/\mkern-5mu/}% \scriptstyle
    {/\mkern-5mu/}}}% \scriptscriptstyle


\usepackage{datenumber}
\usepackage{calc}
\newcounter{datetoday}
\newcounter{diffyears}
\newcounter{diffmonths}
\newcounter{diffdays}
\newcommand{\difftoday}[3]{%
      \setmydatenumber{datetoday}{\the\year}{\the\month}{\the\day}%
      \setmydatenumber{diffdays}{#1}{#2}{#3}%
      \addtocounter{diffdays}{-\thedatetoday}%
      \ifnum\value{diffdays}>0
        \def\diffbefore{Only }%
        \def\diffafter{left}%
      \else
        \def\diffbefore{}%
        \def\diffafter{ago}%
        \setcounter{diffdays}{-\value{diffdays}}%
      \fi
      \setcounter{diffyears}{\value{diffdays}/365}%
      \setcounter{diffdays}{\value{diffdays}-365*\value{diffyears}}%
      \setcounter{diffmonths}{\value{diffdays}/30}%
      \setcounter{diffdays}{\value{diffdays}-30*\value{diffmonths}}%
      %
      \diffbefore
      \ifnum\value{diffyears}=0
      \else
        \ifnum\value{diffyears}>1
            {\color{red}\thediffyears\space years},
        \else
            {\color{red}\thediffyears\space year},
        \fi
      \fi
      \ifnum\value{diffmonths}=0
      \else
        \ifnum\value{diffmonths}>1
            {\color{red}\thediffmonths\space months}
        \else
            {\color{red}\thediffmonths\space month}
        \fi
      \fi
      {\color{red}\thediffdays\space days}
      \diffafter
}

\usepackage[scr=boondoxo]{mathalfa}

\usepackage{tikz}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathmorphing}
\tikzset{snake it/.style={decorate, decoration=snake}}

\DeclareMathAlphabet{\mathpzc}{T1}{pzc}{m}{it}

\def\rcurs{{\mbox{$\resizebox{.09in}{.08in}{\includegraphics[trim= 1em 0 14em 0,clip]{ScriptR}}$}}}
\def\brcurs{{\mbox{$\resizebox{.09in}{.08in}{\includegraphics[trim= 1em 0 14em 0,clip]{BoldR}}$}}}
\def\hrcurs{{\mbox{$\hat \rcurs$}}}

\def\WW{\mathbb{W}}
\def\tWW{\widetilde{\WW}}
\def\hWW{\widehat{\WW}}
\def\VV{\mathbb{V}}
\def\tVV{\widetilde{\VV}}
\def\hVV{\widehat{\VV}}
\newcommand*{\mat}[1]{#1}
\newcommand{\matx}[1]{{\bf #1}} %SY 
\newcommand{\vecc}[1]{{\bf #1}}

\newcommand{\win}[1]{X_{{#1}}}
\newcommand{\game}[1]{\mathsf{G}_{{#1}}}
\newcommand{\hame}[1]{\mathsf{H}_{{#1}}}
\newcommand{\came}[1]{\mathsf{C}_{{#1}}}
\newcommand{\prob}[1]{\mathrm{Pr}\left[{#1}\right]}

\def\ntrp{\omega(\log\ \lambda)}

% \def\B{\mathbf{B}}
% \def\tB{\widetilde{\mathbf{B}}}

% \def\Az{\A_0}
% \def\Ao{\A_1}
% \def\Bz{\B_0}
% \def\Bo{\B_1}
%\def\Bt{\B_2}
% \def\Br{\B_3}
% \def\Bso{\B_1^*}
% \def\Bst{\B_2^*}
% \def\Bsr{\B_3^*}

% \def\Bio{\B_{i,1}}
% \def\Bit{\B_{i,2}}
% \def\Bir{\B_{i,3}}
% \def\Biso{\B_{i,1}^*}
% \def\Bist{\B_{i,2}^*}
% \def\Bisr{\B_{i,3}^*}

% \def\tBo{\tB_1}
% \def\tBt{\tB_2}
% \def\tBr{\tB_3}
% \def\tBso{\tB_1^*}
% \def\tBst{\tB_2^*}
% \def\tBsr{\tB_3^*}

% %\def\v{\mathbf{v}}
% \newcommand{\hv}[1][]{\widehat{v}_{#1}}
% \newcommand{\tv}[1][]{\widetilde{v}_{#1}}
% %\def\tv{\widetilde{v}}
% \def\vo{\v^{(1)}}
% \def\vt{\v^{(2)}}
% \def\vr{\v^{(3)}}
% \def\hvo{\hv^{(1)}}
% \def\hvt{\hv^{(2)}}
% \def\hvr{\hv^{(3)}}
% \def\tvo{\tv^{(1)}}
% \def\tvt{\tv^{(2)}}
% \def\tvr{\tv^{(3)}}

% \def\w{\mathbf{w}}
% \def\wo{\w^{(1)}}
% \def\wt{\w^{(2)}}
% \def\wr{\w^{(3)}}
% \def\twr{\widetilde{\w}^{(3)}}


\def\io{\iota}
\def\pe{\mathsf{ABE}}
\def\ABGgen{\mathcal{G}_{\sf abg}}
\def\FunPriv{\mathsf{FPriv}}
\newcommand*{\wIdCPA}{\mathsf{wID{\mathchar`-}CPA}}
\newcommand*{\IdCPA}{\mathsf{ID{\mathchar`-}CPA}}

\newcommand*{\IndCPA}{\mathsf{IND{\mathchar`-}ID{\mathchar`-}CPA}}
\newcommand*{\IndwIdCPA}{a\mathsf{IND{\mathchar`-}wID{\mathchar`-}CPA}}
\newcommand{\IndIdCPA}{a\mathsf{IND{\mathchar`-}ID{\mathchar`-}CPA}}
\newcommand*{\IndIdCCA}{a\mathsf{IND{\mathchar`-}ID{\mathchar`-}CCA}} %SB
\def\qd{Q}
\def\qq{Q}
\def\qqq{\tilde{Q}}

\def\iseq{\overset{?}{=}}

\newcommand{\Wk}[1][(m,n)]{\mathcal{W}_{#1}}
\newcommand{\Dk}[1][k]{\mathcal{U}_{#1}}
\newcommand{\Fk}[1][n]{\mathcal{F}_{#1}}
\newcommand{\Uk}[1][k]{\mathcal{D}_{#1}}

% changed for SnP Submission
% \newcommand{\matDH}[1][k]{\Dk[#1]\mhyf\mathsf{matDH}}
% \newcommand{\EmatDH}[1][{m,n}]{(#1)\mhyf\mathsf{mE}\mhyf\mathsf{matDH}}
% \newcommand{\kerDH}[1][k]{\Dk[#1]\mhyf\mathsf{kerDH}}
% \newcommand{\bmatDH}[1][k]{bil\mhyf\Dk[#1]\mhyf\mathsf{matDH}}
% \newcommand{\lmatDH}[1][k]{lat\mhyf\Dk[#1]\mhyf\mathsf{matDH}}
% \newcommand{\mbmatDH}[1][k]{m\mhyf bil\mhyf\Dk[#1]\mhyf\mathsf{matDH}}
% \newcommand{\bkerDH}[1][k]{bil\mhyf\Dk[#1]\mhyf\mathsf{kerDH}}
% changed for SnP Submission

\newcommand{\matDH}[1][k]{\Dk[#1]\mhyf\mathsf{MDDH}}
\newcommand{\EmatDH}[1][{m,n}]{(#1)\mhyf\mathsf{mE}\mhyf\mathsf{MDDH}}
\newcommand{\kerDH}[1][k]{\Dk[#1]\mhyf\mathsf{KDH}}
\newcommand{\bmatDH}[1][k]{bil\mhyf\Dk[#1]\mhyf\mathsf{MDDH}}
\newcommand{\lmatDH}[1][k]{lat\mhyf\Dk[#1]\mhyf\mathsf{MDDH}}
\newcommand{\mbmatDH}[1][k]{m\mhyf bil\mhyf\Dk[#1]\mhyf\mathsf{MDDH}}
\newcommand{\bkerDH}[1][k]{bil\mhyf\Dk[#1]\mhyf\mathsf{KDH}}


\newcommand{\EDDH}[1][n]{{#1}\mhyf\mathsf{mE}\mhyf\mathsf{DDH}}
\newcommand{\ddh}{\mathsf{DDH}}
\newcommand{\ddhCan}{\mathsf{DDH}\mhyf\mathsf{II}}

\newcommand{\Dtk}{\mathcal{D}_{2k,k}}
\newcommand{\Dtok}{\mathcal{D}_{2k+1,k}}
\newcommand{\mattDH}{\Dtk\mhyf\mathsf{matDH}}
\def\ppt{\mathsf{ppt}}
\def\cons{\mathcal{P}}
\def\QCr{{\color{\confcolor}Q_{\Cr}}}
\def\QChl{{\color{\confcolor}Q_{\Chl}}}
\def\QTg{{\color{\confcolor}Q_{\Tg}}}
\def\QSk{{\color{\confcolor}Q_{\Sk}}}
\def\SSk{{\color{\confcolor}S_{\Sk}}}
\def\Qsk{{\color{\confcolor}Q_{\sk}}}
\def\Osk{{\color{\confcolor}O_{\sk}}}
\def\Qct{{\color{\confcolor}Q_{\Ct}}}
\def\Oct{{\color{\confcolor}O_{\Ct}}}
\def\Qtrp{{\color{\confcolor}Q_{\Trp}}}
\def\Otrp{{\color{\confcolor}O_{\Trp}}}
\def\Qpk{{\color{\confcolor}Q_{\pk}}}
\def\Opk{{\color{\confcolor}O_{\pk}}}
\def\Qkeys{{\color{\confcolor}Q_{keys}}}
\def\Okeys{{\color{\confcolor}O_{keys}}}
\def\Skeys{{\color{\confcolor}S_{keys}}}

\def\aperp{\matx{a}^\perp}
\def\aperpt{\Apt}
\def\bperp{\matx{b}^\perp}
\def\bperpt{\matx{b}^{\perp^\top}}


\def\AltKgen{\mathsf{AltKeyGen}}			% AKgen
\def\AltDec{\mathsf{AltDecrypt}}			% ADec

\def\sfSetup{\mathsf{SFSetup}}
\def\sfKgen{\mathsf{SFKeyGen}}
\def\sfTgen{\mathsf{sfTrapdoor}}
\def\sfEnc{\mathsf{SFEncrypt}}
\def\sfSEnc{\mathsf{sfSrchEnc}}
\def\sfDec{\mathsf{SFDecrypt}}
\def\sfAltKgen{\mathsf{SFAltKeyGen}}		% sfAKgen
\def\sfAltDec{\mathsf{SFAltDecrypt}}		% sfADec


% \def\TK{\mathbf{tk}}
% \def\AK{\mathbf{AK}}
% \newcommand{\tk}[1][]{\mathsf{tk}_{{#1}}}
% \newcommand{\ak}[1][]{\mathsf{ak}_{{#1}}}

% \newcommand{\U}{\matx{U}}
% \newcommand{\tU}{\widetilde{\matx{U}}}
% \newcommand{\hU}{\hat{\matx{U}}}
% %\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
% \newcommand{\Ut}{\matx{U}^{\top}}
% \newcommand{\tUt}{\widetilde{\matx{U}}^{\top}}
% \newcommand{\hUt}{\hat{\matx{U}}^{\top}}
% %\newcommand{\thWt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\UR}[1][]{\matx{U}_{\Rcvr_{#1}}}
% \newcommand{\tUR}[1][]{\widetilde{\matx{U}}_{\Rcvr_{#1}}}
% \newcommand{\hUR}[1][]{\hat{\matx{U}}_{\Rcvr_{#1}}}
% %\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
% \newcommand{\URt}[1][]{\matx{U}_{\Rcvr_{#1}}^{\top}}
% \newcommand{\tURt}[1][]{\widetilde{\matx{U}}_{\Rcvr_{#1}}^{\top}}
% \newcommand{\hURt}[1][]{\hat{\matx{U}_{\Rcvr_{#1}}}^{\top}}
% %\newcommand{\thWt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\US}{\matx{U}_{\Sndr}}
% \newcommand{\tUS}{\widetilde{\matx{U}}_{\Sndr}}
% \newcommand{\hUS}{\hat{\matx{U}}_{\Sndr}}
% %\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
% \newcommand{\USt}{\matx{U}_{\Sndr}^{\top}}
% \newcommand{\tUSt}{\widetilde{\matx{U}}_{\Sndr}^{\top}}
% \newcommand{\hUSt}{\hat{\matx{U}}_{\Sndr}^{\top}}
% %\newcommand{\thWt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\V}{\matx{V}}
% \newcommand{\tV}{\tilde{\matx{V}}}
% \newcommand{\hV}{\hat{\matx{V}}}
% %\newcommand{\thV}[1]{\tilde{{\matx{V}}}}
% \newcommand{\Vt}{\matx{V}^{\top}}
% \newcommand{\tVt}{\tilde{\matx{V}}^{\top}}
% \newcommand{\hVt}{\hat{\matx{V}}^{\top}}
% %\newcommand{\thVt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\huS}[1][]{{\color{black}\widetilde{u}_{\Sndr_{#1}}}}
% \newcommand{\huSt}[1][]{{\color{black}\widetilde{u}_{\Sndr_{#1}}^\top}}

% \newcommand{\tvR}[1][]{{\color{black}\widetilde{v}_{\Rcvr}^{#1}}}

% \newcommand{\hvR}[1][]{{\color{black}\widehat{v}_{\Rcvr_{#1}}}}
% \newcommand{\hvRt}[1][]{{\color{black}\widehat{v}_{\Rcvr_{#1}}^\top}}


% \newcommand{\VR}[1][]{\matx{V}_{\Rcvr_{#1}}}
% \newcommand{\tVR}[1][]{\tilde{\matx{V}}_{\Rcvr_{#1}}}
% \newcommand{\hVR}[1][]{\hat{\matx{V}}_{\Rcvr_{#1}}}
% %\newcommand{\thV}[1]{\tilde{{\matx{V}}}}
% \newcommand{\VRt}[1][]{\matx{V}_{\Rcvr_{#1}}^{\top}}
% \newcommand{\tVRt}[1][]{\tilde{\matx{V}}_{\Rcvr_{#1}}^{\top}}
% \newcommand{\hVRt}[1][]{\hat{\matx{V}}_{\Rcvr_{#1}}^{\top}}
% %\newcommand{\thVt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\VS}{\matx{V}_{\Sndr}}
% \newcommand{\tVS}{\widetilde{\matx{V}}_{\Sndr}}
% \newcommand{\hVS}{\hat{\matx{V}}_{\Sndr}}
% %\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
% \newcommand{\VSt}{\matx{V}_{\Sndr}^{\top}}
% \newcommand{\tVSt}{\widetilde{\matx{V}}_{\Sndr}^{\top}}
% \newcommand{\hVSt}{\hat{\matx{V}}_{\Sndr}^{\top}}
% %\newcommand{\thWt}[1]{\tilde{{\matx{V}}}^{\top}}

% \newcommand{\x}[1][]{\matx{b}_{{#1}}}
% % \newcommand{\tz}[1][]{\widetilde{\matx{Z}}_{{#1}}}
% % \newcommand{\hZ}[1][]{\hat{\matx{Z}}_{{#1}}}
% \newcommand{\xt}[1][]{\matx{b}_{{#1}}^{\top}}
% % \newcommand{\tZt}[1][]{\widetilde{\matx{Z}}_{{#1}}^{\top}}
% % \newcommand{\hZt}[1][]{\hat{\matx{Z}}_{{#1}}^{\top}}
% \newcommand{\y}[1][]{\matx{d}_{{#1}}}
% % \newcommand{\tZ}[1][]{\widetilde{\matx{Z}}_{{#1}}}
% % \newcommand{\hZ}[1][]{\hat{\matx{Z}}_{{#1}}}
% \newcommand{\yt}[1][]{\matx{d}_{{#1}}^{\top}}
% % \newcommand{\tZt}[1][]{\widetilde{\matx{Z}}_{{#1}}^{\top}}
% % \newcommand{\hZt}[1][]{\hat{\matx{Z}}_{{#1}}^{\top}}

\renewcommand{\a}[1][]{\vecc{h}_{{#1}}}
\newcommand{\at}[1][]{\vecc{h}_{{#1}}^{\top}}
\newcommand{\ta}[1][]{\widetilde{\vecc{h}}_{{#1}}}
\newcommand{\tat}[1][]{\widetilde{\vecc{h}}_{{#1}}^{\top}}

\renewcommand{\d}[1][]{\vecc{t}_{{#1}}}
\newcommand{\dt}[1][]{\vecc{t}_{{#1}}^{\top}}
\newcommand{\td}[1][]{\widetilde{\vecc{t}}_{{#1}}}
\newcommand{\tdt}[1][]{\widetilde{\vecc{t}}_{{#1}}^{\top}}

\renewcommand{\u}[1][]{\vecc{t}_{{#1}}}
\newcommand{\ut}[1][]{\vecc{t}_{{#1}}^{\top}}
% \newcommand{\tu}[1][]{\widetilde{\vecc{t}}_{{#1}}}
% \newcommand{\tut}[1][]{\widetilde{\vecc{t}}_{{#1}}^{\top}}
\newcommand{\tu}[1][]{\widetilde{u}_{#1}}
\newcommand{\tk}[1][]{\widetilde{k}_{#1}}

\newcommand{\z}[1][]{\vecc{z}_{{#1}}}
\newcommand{\zt}[1][]{\vecc{z}_{{#1}}^{\top}}
\newcommand{\tz}[1][]{\widetilde{\vecc{z}}_{{#1}}}
\newcommand{\tzt}[1][]{\widetilde{\vecc{z}}_{{#1}}^{\top}}

% \newcommand{\h}[1][]{\vecc{h}_{{#1}}}
% \renewcommand{\ht}[1][]{\h_{{#1}}^{\top}}
% \renewcommand{\th}[1][]{\widetilde{\h}_{{#1}}}
% \newcommand{\tht}[1][]{\widetilde{\h}_{{#1}}^{\top}}

\def\amsk{{\color{red}\alpha}}
\newcommand{\Amsk}[1][]{\pmb{\amsk}_{{#1}}}
\newcommand{\Amskt}[1][]{\pmb{\amsk}_{{#1}}^{\top}}
\newcommand{\tAmsk}[1][]{\widetilde{\pmb{\amsk}}_{{#1}}}
\newcommand{\tAmskt}[1][]{\widetilde{\pmb{\amsk}}_{{#1}}^{\top}}

\def\bmsk{{\color{red}\beta}}
\newcommand{\Bmsk}[1][]{\pmb{\bmsk}_{{#1}}}
\newcommand{\Bmskt}[1][]{\pmb{\bmsk}_{{#1}}^{\top}}
\newcommand{\tBmsk}[1][]{\widetilde{\pmb{\bmsk}}_{{#1}}}
\newcommand{\tBmskt}[1][]{\widetilde{\pmb{\bmsk}}_{{#1}}^{\top}}

% \def\Amskt{\Amsk^\top}
% \def\tAmsk{\widetilde{\Amsk}}
% \def\tAmskt{\widetilde{\Amsk}^\top}
\newcommand{\J}[1][]{\matx{J}_{{#1}}}
\newcommand{\Jt}[1][]{\matx{J}_{{#1}}^{\top}}
\newcommand{\Q}[1][]{\matx{Q}_{{#1}}}
\newcommand{\Qt}[1][]{\matx{Q}_{{#1}}^{\top}}
\newcommand{\N}[1][]{\matx{N}_{{#1}}}
\newcommand{\Nt}[1][]{\matx{N}_{{#1}}^{\top}}
\newcommand{\hN}[1][]{\widehat{\matx{N}}_{{#1}}}
\newcommand{\hNt}[1][]{\widehat{\matx{N}}_{{#1}}^{\top}}

\newcommand{\X}[1][]{\matx{X}_{{#1}}}
\newcommand{\Xt}[1][]{\matx{X}_{{#1}}^{\top}}
\newcommand{\hX}[1][]{\widehat{\matx{X}}_{{#1}}}
\newcommand{\hXt}[1][]{\widehat{\matx{X}}_{{#1}}^{\top}}
\newcommand{\bX}[1][]{\overline{\matx{X}}_{{#1}}}
\newcommand{\bXt}[1][]{\overline{\matx{X}}_{{#1}}^{\top}}
\newcommand{\Y}[1][]{\matx{Y}_{{#1}}}
\newcommand{\Yt}[1][]{\matx{Y}_{{#1}}^{\top}}
\newcommand{\bY}[1][]{\overline{\matx{Y}}_{{#1}}}
\newcommand{\bYt}[1][]{\overline{\matx{Y}}_{{#1}}^{\top}}
\newcommand{\x}[1][]{\matx{x}_{{#1}}}
\newcommand{\xt}[1][]{\matx{x}_{{#1}}^{\top}}
\newcommand{\txt}[1][]{\widetilde{\matx{x}}_{{#1}}^{\top}}
\newcommand{\y}[1][]{\matx{y}_{{#1}}}
\newcommand{\yt}[1][]{\matx{y}_{{#1}}^{\top}}

\newcommand{\Z}[1][]{\matx{Z}_{{#1}}}
\newcommand{\Zt}[1][]{\matx{Z}_{{#1}}^{\top}}
\newcommand{\hZ}[1][]{\widehat{\matx{Z}}_{{#1}}}
\newcommand{\hZt}[1][]{\widehat{\matx{Z}}_{{#1}}^{\top}}

\newcommand{\D}[1][]{\matx{D}_{{#1}}}
\newcommand{\bD}[1][]{\overline{\matx{D}}_{{#1}}}
\newcommand{\tD}[1][]{\widetilde{\matx{D}}_{{#1}}}
\newcommand{\hD}[1][]{\widehat{\matx{D}}_{{#1}}}
%\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
\newcommand{\Dt}[1][]{\matx{D}_{{#1}}^{\top}}
\newcommand{\bDt}[1][]{\overline{\matx{D}}_{{#1}}^{\top}}
\newcommand{\tDt}[1][]{\widetilde{\matx{D}}_{{#1}}^{\top}}
\newcommand{\hDt}[1][]{\widehat{\matx{D}}_{{#1}}^{\top}}
%\newcommand{\thWt}[1]{\tilde{{\matx{V}}}_{#1}^{\top}}

\newcommand{\U}[1][]{\matx{U}_{{#1}}}
\newcommand{\bU}[1][]{\overline{\matx{U}}_{{#1}}}
\newcommand{\tU}[1][]{\widetilde{\matx{U}}_{{#1}}}
\newcommand{\hU}[1][]{\widehat{\matx{U}}_{{#1}}}
%\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
\newcommand{\Ut}[1][]{\matx{U}_{{#1}}^{\top}}
\newcommand{\bUt}[1][]{\overline{\matx{U}}_{{#1}}^{\top}}
\newcommand{\tUt}[1][]{\widetilde{\matx{U}}_{{#1}}^{\top}}
\newcommand{\hUt}[1][]{\widehat{\matx{U}}_{{#1}}^{\top}}
%\newcommand{\thWt}[1]{\tilde{{\matx{V}}}_{#1}^{\top}}

\renewcommand{\v}[1][]{\vecc{v}_{{#1}}}
\newcommand{\vt}[1][]{\matx{v}_{{#1}}^{\top}}
\newcommand{\tv}[1][]{\widetilde{{v}}_{{#1}}}
%\newcommand{\tvt}[1][]{\widetilde{{v}}_{{#1}}^{\top}}
\newcommand{\V}[1][]{\matx{V}_{{#1}}}
\newcommand{\bV}[1][]{\overline{\matx{V}}_{{#1}}}
\newcommand{\tV}[1][]{\widetilde{\matx{V}}_{{#1}}}
\newcommand{\hV}[1][]{\widehat{\matx{V}}_{{#1}}}
%\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
\newcommand{\Vt}[1][]{\matx{V}_{{#1}}^{\top}}
\newcommand{\bVt}[1][]{\overline{\matx{V}}_{{#1}}^{\top}}
\newcommand{\tVt}[1][]{\widetilde{\matx{V}}_{{#1}}^{\top}}
\newcommand{\hVt}[1][]{\widehat{\matx{V}}_{{#1}}^{\top}}
%\newcommand{\thWt}[1]{\tilde{{\matx{V}}}_{#1}^{\top}}

\newcommand{\w}[1][]{\vecc{w}_{{#1}}}
\newcommand{\bw}[1][]{\overline{\vecc{w}}_{{#1}}}
\newcommand{\W}[1][]{\matx{W}_{{#1}}}
\newcommand{\tW}[1][]{\widetilde{\matx{W}}_{{#1}}}
\newcommand{\hW}[1][]{\widehat{\matx{W}}_{{#1}}}
%\newcommand{\thW}[1]{\tilde{{\matx{V}}}_{#1}}
\newcommand{\wt}[1][]{\vecc{w}_{{#1}}^{\top}}
\newcommand{\bwt}[1][]{\overline{\vecc{w}}_{{#1}}^{\top}}
\newcommand{\Wt}[1][]{\matx{W}_{{#1}}^{\top}}
\newcommand{\tWt}[1][]{\widetilde{\matx{W}}_{{#1}}^{\top}}
\newcommand{\hWt}[1][]{\widehat{\matx{W}}_{{#1}}^{\top}}
%\newcommand{\thWt}[1]{\tilde{{\matx{V}}}_{#1}^{\top}}

\newcommand{\K}[1][]{\matx{K}_{{#1}}}
\newcommand{\Kt}[1][]{\matx{K}_{{#1}}^{\top}}
\newcommand{\hK}[1][]{\widehat{\matx{K}}_{{#1}}}
\newcommand{\hKt}[1][]{\widehat{\matx{K}}_{{#1}}^{\top}}
\newcommand{\tK}[1][]{\widetilde{\matx{K}}_{{#1}}}
\newcommand{\tKt}[1][]{\widetilde{\matx{K}}_{{#1}}^{\top}}

\newcommand{\R}[1][]{\matx{R}_{{#1}}}
\newcommand{\Rt}[1][]{\matx{R}_{{#1}}^{\top}}
\newcommand{\hR}[1][]{\widehat{\matx{R}}_{{#1}}}
\newcommand{\hRt}[1][]{\widehat{\matx{R}}_{{#1}}^{\top}}

\newcommand{\f}[1][]{\vecc{f}_{{#1}}}
\newcommand{\ft}[1][]{\matx{f}_{{#1}}^{\top}}
\newcommand{\fu}[1][]{\overline{\vecc{f}}_{{#1}}}
\newcommand{\fut}[1][]{\overline{\matx{f}}_{{#1}}^{\top}}

\newcommand{\A}{\matx{A}}
\newcommand{\At}{\A^{\top}}
\newcommand{\Ap}{\A^{\perp}}
\newcommand{\Apt}{{\Ap}^{\top}}
\newcommand{\Az}{\A_0}
\newcommand{\Azt}{\Az^{\top}}
\newcommand{\Ao}{\A_1}
\newcommand{\Aot}{\Ao^{\top}}
\newcommand{\Azs}{\Az^*}
\newcommand{\Aos}{\Ao^*}

\newcommand{\Au}{\overline{\A}}
\newcommand{\Am}{\underline{\overline{\A}}}
\newcommand{\Ad}{\underline{\A}}
\newcommand{\Aut}{\Au^{\top}}
\newcommand{\Amt}{\Am^{\top}}
\newcommand{\Adt}{\Ad^{\top}}

\newcommand{\Bu}{\overline{\B}}
\newcommand{\Bm}{\underline{\overline{\B}}}
\newcommand{\Bd}{\underline{\B}}
\newcommand{\But}{\Bu^{\top}}
\newcommand{\Bmt}{\Bm^{\top}}
\newcommand{\Bdt}{\Bd^{\top}}


\newcommand{\B}{\matx{B}}
\newcommand{\Bt}{\B^{\top}}
\newcommand{\Bp}{\B^{\perp}}
\newcommand{\Bpt}{{\Bp}^{\top}}
\newcommand{\Bz}{\B_0}
\newcommand{\Bzt}{\Bz^{\top}}
\newcommand{\Bo}{\B_1}
\newcommand{\Bot}{\Bo^{\top}}
\newcommand{\Bzs}{\Bz^*}
\newcommand{\Bzst}{(\Bz^*)^{\top}}
\newcommand{\Bos}{\Bo^*}
\newcommand{\Bost}{(\Bo^*)^{\top}}

\newcommand{\M}{\matx{D}}
\newcommand{\Mt}{\M^{\top}}
\newcommand{\Mp}{\M^{\perp}}
\newcommand{\Mpt}{{\Mp}^{\top}}
\newcommand{\Mz}{\M_0}
\newcommand{\Mzt}{\Mz^{\top}}
\newcommand{\Mo}{\M_1}
\newcommand{\Mot}{\Mo^{\top}}
\newcommand{\Mzs}{\Mz^*}
\newcommand{\Mos}{\Mo^*}
\newcommand{\Mu}{\overline{\M}}
\newcommand{\Mm}{\underline{\overline{\M}}}
\newcommand{\Md}{\underline{\M}}
\newcommand{\Mut}{\Mu^{\top}}
\newcommand{\Mmt}{\Mm^{\top}}
\newcommand{\Mdt}{\Md^{\top}}

\newcommand{\F}[1][]{\matx{F}_{{#1}}}
\newcommand{\Ft}[1][]{\F_{{#1}}^{\top}}
\newcommand{\Fu}[1][]{\overline{\F}_{{#1}}}
\newcommand{\Fm}[1][]{\underline{\overline{\F}}_{{#1}}}
\newcommand{\Fd}[1][]{\underline{\F}_{{#1}}}
\newcommand{\Fut}[1][]{\Fu_{{#1}}^{\top}}
\newcommand{\Fmt}[1][]{\Fm_{{#1}}^{\top}}
\newcommand{\Fdt}[1][]{\Fd_{{#1}}^{\top}}


\def\bS{\overline{\mathbf{S}}}
\def\S{\mathbf{S}}
%\def\s{\mathbf{s}}
\def\St{\S^\top}
\def\st{\s^\top}
\newcommand{\s}[1][]{\vecc{s}_{{#1}}}


% \def\z{\mathbf{z}}
% \def\hz{\widehat{\z}}
% \def\tz{\widetilde{\z}}
% \def\zt{\z^\top}
% \def\hzt{\hz^\top}
% \def\tzt{\tz^\top}

\def\ts{\widetilde{\s}}
\def\tst{\ts^\top}
\def\tr{\widetilde{\r}}
\def\trt{\tr^\top}

\def\hs{\widehat{s}}
\def\hr{\widehat{r}}


\def\bR{\overline{\mathbf{R}}}
%\def\R{\mathbf{R}}
\def\r{\mathbf{r}}
% \def\Rt{\R^\top}
\def\rt{\r^\top}

% \def\bU{\overline{\mathbf{U}}}
% \def\U{\mathbf{U}}
% \def\u{\mathbf{u}}
% %\def\Ut{\U^\top}
% \def\ut{\u^\top}

\def\bT{\overline{\mathbf{T}}}
\def\T{\mathbf{T}}
\def\t{\mathbf{t}}




\def\hu{\overline{\matx{h}}}
\def\hd{\underline{\matx{h}}}

% \newcommand{\hu}[1][]{\widehat{u}_{#1}}
\def\sample{\hookleftarrow}
%\def\sample{\overset{\$}{\leftarrow}}

\def\C{\matx{C}}
%\def\V{\matx{V}}
% \def\Y{\matx{Y}}
% \def\Z{\matx{Z}}

% \def\w{\vecc{w}}
% \def\wo{\w^{(1)}}
% \def\wt{\w^{(2)}}
% \def\wr{\w^{(3)}}

%\newcommand{\K}{\matx{K}}
% \newcommand{\hK}{\hat{K}}
\def\e{\vecc{e}}
\def\t{\vecc{t}}
\def\c{\vecc{c}}
%\def\u{\vecc{u}}
%\def\v{\vecc{v}}
%\def\h{\vecc{h}}
\def\k{\vecc{k}}
% \def\s{\vecc{s}}
% \def\r{\vecc{r}}
% \def\x{\vecc{x}}
% \def\y{\vecc{y}}
%\def\z{\vecc{z}}
%\def\hr{\hat{\vecc{r}}}
\def\Ffnc{\mathcal{F}}
\def\Hfnc{\mathcal{H}}
\newcommand{\iCol}[2]{\left(\begin{matrix}#1\\#2\end{matrix}\right)}
%\newcommand{\iRow}[2]{\left(\begin{matrix}#1&#2\\\end{matrix}\right)}
\newcommand{\iRow}[2]{\left(#1\parallel #2\right)}
\newcommand{\iMat}[4]{\left(\begin{matrix}#1&#2\\#3&#4\end{matrix}\right)}
\newcommand{\Sumn}[2]{\sum\limits_{\substack{#1\notin #2}}}
\newcommand{\Sum}[2]{\sum\limits_{\substack{#1\in #2}}}
\newcommand{\Sumeq}[4]{\sum\limits_{\substack{#1\in #2\\ #3=#4}}}
\newcommand{\Sumneq}[4]{\sum\limits_{\substack{#1\in #2\\ #3\neq #4}}}
\newcommand{\Summ}[4]{\sum\limits_{\substack{#1\in #2\\ #3\in #4}}}
\newcommand{\Prod}[2]{\prod\limits_{\substack{#1\in #2}}}
\newcommand{\Prodd}[4]{\prod\limits_{\substack{#1\in #2\\ #3\in #4}}}

\newcommand{\SumiDT}[3][i]{\sum_{#1=#2}^{#3}}
\newcommand{\SumniDT}[4][i]{\sum_{\begin{matrix}
  #1=#2\\
  #1\neq #4\\
\end{matrix}}^{#3}}

\def\abG{\mathcal{G}}
\def\ABSGen{\mathsf{ABSGen}}
\def\go{g_1}
\def\gt{g_2}
\def\gT{g_{\text{T}}}
\def\Go{\mathbb{G}_1}						% \sG = \Go^{k+1}
\def\Gt{\mathbb{G}_2}						% \sH = \Gt^{k+1}
\def\GT{\mathbb{G}_{\text{T}}}				% \GT = \Gr
\newcommand{\GGp}{\mathsf{G_p}}
\newcommand{\GGe}{\mathsf{G_e}}
\def\SzZp{|\Zp|}
\def\SzGo{|\Go|}
\def\SzGt{|\Gt|}
\def\SzGT{|\GT|}

\def\AA{\mathcal{A}}
\def\AC{\mathcal{C}}
\def\AB{\mathcal{B}}

\def\secpp{\lambda}
\newcommand{\adv}[2]{\mathsf{Adv}_{#1}^{#2}(\secpp)}
\newcommand{\Adv}[2]{{\mathsf{Adv}_{#1}^{#2}(\secpp)}}
\newcommand{\Exp}[3]{\mathsf{Exp}_{#1}^{#2}(\secpp\ifthenelse{\equal{#3}{}}{}{,#3})}
\newcommand{\neglgbl}[1][\secpp]{\mathsf{neg}(#1)}
\newcommand{\poly}[1][\secpp]{\mathsf{poly}(#1)}

\def\plc{\mathsf{P}}
\def\Zp{\mathbb{Z}_p}

% \setlength{\textwidth}{6in}
% \setlength{\textheight}{9in}
% \setlength{\parskip}{4pt}
% \hoffset=-0.5in
% \voffset=-0.7in

%\newcommand{\icol}[2]{\big(\begin{smallmatrix}#1\\#2\end{smallmatrix}\big)}
%\newcommand{\irow}[2]{\left(\begin{smallmatrix}#1&#2\end{smallmatrix}\right)}
%\newcommand{\iCol}[2]{\left(\begin{matrix}#1\\#2\end{matrix}\right)}
%\newcommand{\iRow}[2]{\left(\begin{matrix}#1&#2\end{matrix}\right)}

% group one or two
% Changed for SnP
% \newcommand{\Gp}[1]{\left\llbracket #1\right\rrbracket}
% \newcommand{\On}[1]{\left\llbracket #1\right\rrbracket_1}
% \newcommand{\Tw}[1]{\left\llbracket #1\right\rrbracket_2}
% \newcommand{\Tt}[1]{\left\llbracket #1\right\rrbracket_\textrm{T}}
% Changed for SnP

\newcommand{\Gp}[1]{\left[ #1\right]}
\newcommand{\On}[1]{\left[ #1\right]_1}
\newcommand{\Tw}[1]{\left[ #1\right]_2}
\newcommand{\Tt}[1]{\left[ #1\right]_\textrm{T}}

% Changed for SnP
% \def\bee{\mathfrak{b}}
% Changed for SnP


\def\aaa{\mathscr{a}}
\def\bee{\mathscr{b}}
\def\cee{\mathscr{c}}
\def\dee{\mathscr{d}}
\def\eee{\mathscr{e}}
\def\ef{\mathscr{f}}
\def\gee{\mathscr{g}}
\def\eich{\mathscr{h}}
%\def\eich{2k}
\def\kay{\mathscr{k}}								% caligraphic k
\def\el{\mathscr{l}}								% caligraphic k
\def\tee{\mathscr{t}}
%\def\tee{k}
\def\enn{\mathscr{n}}
\def\emm{\mathscr{m}}
\def\es{\mathscr{s}}
\def\ar{\mathscr{r}}
\def\eu{\mathscr{u}}
\def\veee{\mathscr{v}}
\def\wee{\mathscr{w}}
\def\zee{\mathscr{z}}
\def\ii{\iota}
\def\ij{\jmath}

\def\SetuP{\mathbf{Setup}}
\def\QPhase#1{\mathbf{Query\ Phase}\text{-}{\sf #1}}
\def\KeyQ{\mathbf{Key\ Queries}}
\def\EncQ{\mathbf{Enc\ Queries}}
\def\DecQ{\mathbf{Dec\ Queries}}
\def\CorQ{\mathbf{Cor\ Queries}}
\def\Chal{\mathbf{Challenge}}
\def\Guess{\mathbf{Guess}}
\def\IniT{\mathbf{Init}}
\def\Correct{\mathbf{Correctness}.}
\def\TrpQ{\mathbf{Trapdoor\ Queries}}
\def\Forge{\mathbf{Forge}}

% changed for SnP Submission
% \def\Setup{\mathsf{Setup}}
% \def\Kgen{\mathsf{KeyGen}}
% \def\SEnc{\mathsf{SrchEnc}}
% \def\Tgen{\mathsf{Trapdoor}}
% \def\Test{\mathsf{Test}}
% changed for SnP Submission
\def\Setup{\textsc{Setup}}
\def\Kgen{\textsc{KeyGen}}
\def\SEnc{\textsc{SrchEnc}}
\def\Tgen{\textsc{TrapGen}}
\def\Test{\textsc{Test}}

\def\XEval{\mathsf{XEval}}
\def\YEval{\mathsf{YEval}}
\def\Update{\mathsf{Update}}
\def\Rand{\mathsf{ReSign}}
\def\Verif{\mathsf{Verify}}
\def\Gen{\mathsf{Gen}}
\def\Init{\mathsf{Init}}
\def\AKgen{\mathsf{AltKeyGen}}
\def\Enc{\mathsf{Encrypt}}
\def\Dec{\mathsf{Decrypt}}
\def\ADec{\mathsf{AltDecrypt}}
\def\msk{\mathsf{msk}}
\def\mpk{\mathsf{mpk}}
\def\ppC{\mathsf{params}}
\def\pp{\mathsf{pp}}
\def\hpk{\widehat{\pk}}
\def\pk{\mathsf{pk}}
\def\PK{\mathsf{PK}}
\def\chpk{\mathsf{pk}^*}
\def\hsk{\widehat{\sk}}
\def\sk{\mathsf{sk}}
\def\sky{\mathsf{d}}
\def\chsk{\mathsf{sk}^*}
\def\ssk{{\color{blue}\kappa}}
\def\Ask{\mathbf{ak}}
% \def\ct{\mathbf{c}}
\def\hct{\widehat{\ct}}
\def\ctu{\overline{\ct}}
\def\ctd{\underline{\ct}}
\def\cT{\mathsf{cT}}
\def\Param{\mathsf{Param}}
\def\EncK{\mathsf{EncK}}
\def\EncC{\mathsf{EncC}}
\def\Pair{\mathsf{Pair}}
\def\tmsk{\widetilde{\msk}}
\def\hmsk{\widehat{\msk}}
\def\vrk{\mathsf{vk}}
\def\sgk{\mathsf{sgk}}
\def\Sign{\mathsf{Sign}}
\def\omsk{\mathsf{omsk}}
\def\ompk{\mathsf{ompk}}
\def\ovrk{\mathsf{ovk}}
\def\osgk{\mathsf{osgk}}
\def\Trp{\mathsf{Tr}}
% \def\trp{\mathbf{k}}
\def\Chl{\mathsf{C}}
\def\Cr{\mathsf{Cr}}
% \def\chl{\mathbf{h}}
\def\Tg{\mathsf{T}}
% \def\tg{\mathbf{t}}
\def\trpu{\overline{\trp}}
\def\trpd{\underline{\trp}}
\def\chTrp{\Trp^*}
\def\chtrp{\trp^*}

\newcommand{\chl}[1][]{\mathbf{c}_{{#1}}}
\newcommand{\tg}[1][]{\mathbf{t}_{{#1}}}
\newcommand{\ct}[1][]{\mathbf{ct}_{{#1}}}
\newcommand{\trp}[1][]{\mathbf{k}_{{#1}}}


%\def\TrpQ{\mathbf{Trapdoor\ Queries}}
\newcommand{\Prb}[1]{\Pr\left[#1\right]}

\def\keyrepr{\kay}
\def\Keyrepr{k}
\def\ctrepr{\hat{c}}
\def\Ctrepr{c}
\def\Erepr{E}
\def\Frepr{F}

\newcommand{\ke}[1]{\mathrm{\keyrepr}_{#1}}
\newcommand{\Ke}[1]{\mathrm{\Keyrepr}_{#1}}
\newcommand{\kei}[1]{\mathrm{\keyrepr}'_{#1}}	
\newcommand{\ce}[1]{\mathrm{\ctrepr}_{#1}}
\newcommand{\Ce}[1]{\mathrm{\Ctrepr}_{#1}}
\newcommand{\Ee}[1]{\mathrm{\Erepr}_{#1}}
\newcommand{\Fe}[1]{\mathrm{\Frepr}_{#1}}
\newcommand{\Eei}[1]{\mathrm{\Erepr}'_{#1}}
\def\enck{\mathbf{\Keyrepr}}	% key-encoding
\def\enckl{\pmb{\keyrepr}}	% key-encoding
\def\enckr{\mathbf{\Keyrepr}}	% key-encoding
\def\encc{\mathbf{\Ctrepr}}		% ciphertext-encoding
\def\enccl{\pmb{\ctrepr}}	% key-encoding
\def\enccr{\mathbf{\Ctrepr}}	% key-encoding
\def\pair{\mathbf{\Erepr}}		% pairing matrix
\def\pairt{\mathbf{\Frepr}}		% pairing matrix


\def\keindx{\iota}
\def\ceindx{\tilde{\iota}}

\def\kio{\kappa}
\def\kit{\iota}
\def\cio{\tilde{\kio}}
\def\cit{\tilde{\kit}}

%\def\klen{K}
%
%\def\kleno{m_1}
%\def\klent{m_2}
%\def\klenr{m_3}

% \def\krndn{m_1}
% \def\krndl{m_2}
% \def\klen{m_3}

% \def\kleni{\klen'}

%\def\cle{L}
%\def\cleno{q_1}
%\def\clent{q_2}
%\def\clenr{q_3}

% \def\crndn{q_1}
% \def\crndl{q_2}
% \def\clen{q_3}


%\def\crand{\es}
%\def\krand{\ar}
%\def\krandi{\krand'}	

\def\cmn{w}
%	\newcommand{\pecmn}[1][]{\text{\cmn}_{#1}}
%	\newcommand{\hpecmn}[1][]{\hat{\text{\cmn}}_{#1}}
\newcommand{\pecmn}[1]{\text{\cmn}_{#1}}
\newcommand{\hpecmn}[1]{\hat{\text{\cmn}}_{#1}}
\def\pecmns{\mathbf{\cmn}}
\def\hpecmns{\hat{\pecmns}}

\def\ctrand{s}
\def\cttrand{t}
\def\keyrand{r}
\def\keyyrand{u}

\def\hkyRz{\hat{\mathfrak{r}}_0}
\def\kyRz{\mathfrak{r}_0}
\def\ots{\mathsf{OTS}}
\def\pots{\mathsf{POTS}}


\newcommand{\cts}[1][]{\ctrand_{#1}}
\newcommand{\ctt}[1][]{\cttrand_{#1}}
\newcommand{\kyr}[1][]{\keyrand_{#1}}
\newcommand{\kyu}[1][]{\keyyrand_{#1}}
\newcommand{\hcts}[1][]{\hat{\ctrand}_{#1}}
\newcommand{\hctt}[1][]{\hat{\cttrand}_{#1}}
\newcommand{\hkyr}[1][]{\hat{\keyrand}_{#1}}
\newcommand{\hkyu}[1][]{\hat{\keyyrand}_{#1}}

\newcommand{\ctS}[1][]{\mathbf{\ctrand}_{#1}}
\newcommand{\ctT}[1][]{\mathbf{\cttrand}_{#1}}
\newcommand{\kyR}[1][]{\mathbf{\keyrand}_{#1}}
\newcommand{\kyU}[1][]{\mathbf{\keyyrand}_{#1}}
\newcommand{\hctS}[1][]{\hat{\mathbf{\ctrand}}_{#1}}
\newcommand{\hctT}[1][]{\hat{\mathbf{\cttrand}}_{#1}}
\newcommand{\hkyR}[1][]{\hat{\mathbf{\keyrand}}_{#1}}
\newcommand{\hkyU}[1][]{\hat{\mathbf{\keyyrand}}_{#1}}

\def\CTs{S}
\def\CTt{T}
\def\KYr{R}
\def\KYu{U}
\def\hCTs{\widehat{\rm \CTs}}
\def\hCTt{\widehat{\rm \CTt}}
\def\hKYr{\widehat{\rm \KYr}}
\def\hKYu{\widehat{\rm \KYu}}
\def\CTS{\mathbf{\CTs}}
\def\CTT{\mathbf{\CTt}}
\def\KYR{\mathbf{\KYr}}
\def\KYU{\mathbf{\KYu}}
\def\TCTS{\widetilde{\mathbf{\CTs}}}
\def\TCTT{\widetilde{\mathbf{\CTt}}}
%\newcommand{\ctt}[1][]{\cttrand_{#1}}

\newcommand{\peajk}{a_{\ceindx jk}}
\newcommand{\peajK}{a_{\ceindx jk'}}
\newcommand{\peaJk}{a_{\ceindx j'k}}
\newcommand{\peaJK}{a_{\ceindx j'k'}}
\newcommand{\peAjk}{a_{\ceindx''jk}}
\newcommand{\peaj}{a_{\cit j}}
\newcommand{\lpeaj}{\aaa_{\cio j}}
\newcommand{\peaJ}{a_{\ceindx j'}}


\newcommand{\pebjk}{b_{\keindx jk}}
\newcommand{\pebjK}{b_{\keindx jk'}}
\newcommand{\pebJk}{b_{\keindx j'k}}
\newcommand{\pebJK}{b_{\keindx j'k'}}
\newcommand{\peBjk}{b_{\keindx ''jk}}
\newcommand{\pebj}{b_{\kit j}}
\newcommand{\lpebj}{\bee_{\kio j}}
\newcommand{\pebJ}{b_{\keindx j'}}
\newcommand{\peb}{b_{\keindx}}

\def\Tau{\pmb{\tau}}
\newcommand{\perm}{\tau}
\newcommand{\Perm}[1]{\Gamma^{({#1})}}

\def\GammaW{\pmb{\Gamma}}
\def\GammaV{\pmb{\Lambda}}
%\def\SSk{\mathcal{SSK}}
\def\Sk{\mathsf{K}}
\def\SK{\mathcal{SK}}
\def\TRP{\mathcal{T}}
\def\CT{\mathcal{CT}}
\def\Ct{\mathsf{Ct}}
\def\chCt{\mathsf{Ct}^*}
\def\Ssk{\mathsf{\pmb{\ssk}}}
\def\DtI{\mathcal{Y}}
\def\KyI{\mathcal{X}}
\def\DTi{\mathbf{Y}}
\def\KYi{\mathbf{x}}
\newcommand{\Dti}[1][]{\mathbf{y}_{#1}}
\newcommand{\dti}[1][]{\mathsf{y}_{#1}}	% datai
\newcommand{\kyi}[1][]{\mathsf{x}_{#1}}
%\def\kyi{x}
\def\pfnc{\mathsf{R}}
\def\hfnc{\mathsf{H}}
\def\id{\mathsf{id}}
\def\ID{\mathcal{ID}}
\def\YSet{\mathsf{S}}

\newcommand{\II}[1][]{\mathbb{I}_{{#1}}}


%\def\kw{w}
\def\kw{\omega}
\def\kywd{\tau}
\def\rbtkw{{\kw}'}
%SnP
%SnP
\def\kwd{w}%\tilde{\kw}}
\def\chkw{{\kw}^*}
\def\chkwd{{\tilde{\kw}}^*}
\def\SSet{\mathcal{S}}
\def\chSSet{{\mathcal{S}}^*}
\def\RSet{\mathcal{R}}
\def\chRSet{{\mathcal{R}}^*}
\def\USet{\mathcal{U}}
\def\KWd{\mathcal{KW}}

\def\Users{\mathcal{U}}
\def\Usr{\mathsf{U}}
\def\Usrr{\Usr'}
% Changed for SnP
% \def\Sndr{S}
% \def\Rcvr{R}
% Changed for SnP
% \newcommand{\Rcvr}[1][]{\mathsf{R}^{{#1}}}
\def\Rcvr{\mathsf{R}}
\def\Sndr{\mathsf{S}}
\def\Rcvrr{\mathsf{F}}%\widetilde{\Rcvr}}
\def\Sndrr{\mathsf{E}}%\widetilde{\Sndr}}
\def\chRcvr{{\Rcvr}^*}
\def\chRcvrr{{\Rcvrr}^*}
\def\chSndr{{\Sndr}^*}
\def\chSndrr{{\Sndrr}^*}
\def\rbtRcvr{{\Rcvr}'}
\def\rbtSndr{{\Sndr}'}

\newcommand{\RFdef}[2][\Usr]{\mathsf{RF}_{#2}}
\newcommand{\RF}[3][\Usr]{\RFdef{#2}(#3)}
\newcommand{\ZFdef}[2][\Usr]{\mathsf{ZF}_{#2}}
\newcommand{\ZF}[3][\Usr]{\ZFdef{#2}(#3)}
\newcommand{\OFdef}[2][\Usr]{\mathsf{OF}_{#2}}
\newcommand{\OF}[3][\Usr]{\OFdef{#2}(#3)}
\newcommand{\tZFdef}[2][\Usr]{\widetilde{\mathsf{ZF}}_{#2}}
\newcommand{\tZF}[3][\Usr]{\tZFdef{#2}(#3)}
\newcommand{\tOFdef}[2][\Usr]{\widetilde{\mathsf{OF}}_{#2}}
\newcommand{\tOF}[3][\Usr]{\tOFdef{#2}(#3)}
\newcommand{\SRFdef}[2][\Usr]{\mathsf{RF}_{#2}}
\newcommand{\SRF}[3][\Usr]{\SRFdef{#2}(#3)}
\newcommand{\SZFdef}[2][\Usr]{\mathsf{ZF}_{#2}}
\newcommand{\SZF}[3][\Usr]{\SZFdef{#2}(#3)}
\newcommand{\SOFdef}[2][\Usr]{\mathsf{OF}_{#2}}
\newcommand{\SOF}[3][\Usr]{\SOFdef{#2}(#3)}
\newcommand{\tSZFdef}[2][\Usr]{\widetilde{\mathsf{ZF}}_{#2}}
\newcommand{\tSZF}[3][\Usr]{\tSZFdef{#2}(#3)}
\newcommand{\tSOFdef}[2][\Usr]{\widetilde{\mathsf{OF}}_{#2}}
\newcommand{\tSOF}[3][\Usr]{\tSOFdef{#2}(#3)}
\newcommand{\RRFdef}[2][\Usr]{\mathsf{RF}_{#2}}
\newcommand{\RRF}[3][\Usr]{\RRFdef{#2}(#3)}
\newcommand{\RZFdef}[2][\Usr]{\mathsf{ZF}_{#2}}
\newcommand{\RZF}[3][\Usr]{\RZFdef{#2}(#3)}
\newcommand{\ROFdef}[2][\Usr]{\mathsf{OF}_{#2}}
\newcommand{\ROF}[3][\Usr]{\ROFdef{#2}(#3)}
\newcommand{\tRZFdef}[2][\Usr]{\widetilde{\mathsf{ZF}}_{#2}}
\newcommand{\tRZF}[3][\Usr]{\tRZFdef{#2}(#3)}
\newcommand{\tROFdef}[2][\Usr]{\widetilde{\mathsf{OF}}_{#2}}
\newcommand{\tROF}[3][\Usr]{\tROFdef{#2}(#3)}


% % \newcommand{\RFdef}[2][\Usr]{\mathsf{RF}_{#1,#2}}
% % \newcommand{\RF}[3][\Usr]{\mathsf{RF}_{#1,#2}(#3)}
% \newcommand{\SFdef}[2][\Usr]{\mathsf{SF}_{#2}^{#1}}
% \newcommand{\SF}[3][\Usr]{\mathsf{SF}_{#2}^{#1}(#3)}

% % \newcommand{\RFdef}[2][\Usr]{\mathsf{RF}_{#2}^{#1}}
% \newcommand{\XRFdef}[2][\Usr]{\mathsf{SRF}_{#2}^{#1}}
% \newcommand{\ZRFdef}[2][\Usr]{\mathsf{RRF}_{#2}^{#1}}
% % \newcommand{\RF}[3][\Usr]{\mathsf{RF}_{#2}^{#1}(#3)}

% %\newcommand{\RF}[3][\Usr]{\mathsf{RF}(#1,#3)}
% % \newcommand{\RF}[3]{\mathsf{RF}(#1,#2,#3)}

% % \newcommand{\RF}[3][\Usr]{\mathsf{RF}_{#2}^{#1}(#3)}
% \newcommand{\XRF}[3][\Usr]{\mathsf{SRF}_{#2}^{#1}(#3)}
% \newcommand{\ZRF}[3][\Usr]{\mathsf{RRF}_{#2}^{#1}(#3)}
% \newcommand{\tRFdef}[2][\Usr]{\widetilde{\mathsf{RF}}_{#2}^{#1}}
% \newcommand{\tRF}[3][\Usr]{\widetilde{\mathsf{RF}}_{#2}^{#1}(#3)}
% % \newcommand{\ZFdef}[2][\Usr]{\mathsf{ZF}_{#2}^{#1}}
% \newcommand{\XZFdef}[2][\Usr]{\mathsf{SZF}_{#2}^{#1}}
% \newcommand{\ZZFdef}[2][\Usr]{\mathsf{RZF}_{#2}^{#1}}
% \newcommand{\tXZFdef}[2][\Usr]{\widetilde{\mathsf{SZF}}_{#2}^{#1}}
% \newcommand{\tZZFdef}[2][\Usr]{\widetilde{\mathsf{RZF}}_{#2}^{#1}}
% \newcommand{\LZFdef}[2][\Usr]{\mathsf{LZF}_{#2}^{#1}}
% \newcommand{\RZFdef}[2][\Usr]{\mathsf{RZF}_{#2}^{#1}}
% % \newcommand{\ZF}[3][\Usr]{\mathsf{ZF}_{#2}^{#1}(#3)}
% \newcommand{\XZF}[3][\Usr]{\mathsf{SZF}_{#2}^{#1}(#3)}
% \newcommand{\ZZF}[3][\Usr]{\mathsf{RZF}_{#2}^{#1}(#3)}
% \newcommand{\tXZF}[3][\Usr]{\widetilde{\mathsf{SZF}}_{#2}^{#1}(#3)}
% \newcommand{\tZZF}[3][\Usr]{\widetilde{\mathsf{RZF}}_{#2}^{#1}(#3)}
% \newcommand{\LZF}[3][\Usr]{\mathsf{LZF}_{#2}^{#1}(#3)}
% \newcommand{\RZF}[3][\Usr]{\mathsf{RZF}_{#2}^{#1}(#3)}
% % \newcommand{\tZFdef}[2][\Usr]{\widetilde{\mathsf{ZF}}_{#2}^{#1}}
% % \newcommand{\tZF}[3][\Usr]{\widetilde{\mathsf{ZF}}_{#2}^{#1}(#3)}
% % \newcommand{\OFdef}[2][\Usr]{\mathsf{OF}_{#2}^{#1}}
% \newcommand{\XOFdef}[2][\Usr]{\mathsf{SOF}_{#2}^{#1}}
% \newcommand{\ZOFdef}[2][\Usr]{\mathsf{ROF}_{#2}^{#1}}
% \newcommand{\tXOFdef}[2][\Usr]{\widetilde{\mathsf{SOF}}_{#2}^{#1}}
% \newcommand{\tZOFdef}[2][\Usr]{\widetilde{\mathsf{ROF}}_{#2}^{#1}}
% \newcommand{\LOFdef}[2][\Usr]{\mathsf{LOF}_{#2}^{#1}}
% \newcommand{\ROFdef}[2][\Usr]{\mathsf{ROF}_{#2}^{#1}}
% % \newcommand{\OF}[3][\Usr]{\mathsf{OF}_{#2}^{#1}(#3)}
% \newcommand{\XOF}[3][\Usr]{\mathsf{SOF}_{#2}^{#1}(#3)}
% \newcommand{\ZOF}[3][\Usr]{\mathsf{ROF}_{#2}^{#1}(#3)}
% \newcommand{\tXOF}[3][\Usr]{\widetilde{\mathsf{SOF}}_{#2}^{#1}(#3)}
% \newcommand{\tZOF}[3][\Usr]{\widetilde{\mathsf{ROF}}_{#2}^{#1}(#3)}
% \newcommand{\LOF}[3][\Usr]{\mathsf{LOF}_{#2}^{#1}(#3)}
% \newcommand{\ROF}[3][\Usr]{\mathsf{ROF}_{#2}^{#1}(#3)}
% % \newcommand{\tOFdef}[2][\Usr]{\widetilde{\mathsf{OF}}_{#2}^{#1}}
% % \newcommand{\tOF}[3][\Usr]{\widetilde{\mathsf{OF}}_{#2}^{#1}(#3)}

\newcommand{\msgi}[2][\Msg]{#1_{|#2}}
\newcommand{\msgii}[2][\Msg]{#1_{#2}}
% \newcommand{\msgiii}[2][\Msg]{#1$ $_{#2}}
\def\klen{\alpha}
\def\ulen{\eu}

% Changed for SnP
% \def\paeks{\mathsf{PaEKS}}
% \def\baeks{\mathsf{BaEKS}}
% Changed for SnP
\def\paeks{\textsf{paeks}}
\def\baeks{\textsf{baeks}}

\def\kasae{\mathsf{KASaE}}
\def\OKgen{\mathsf{OKgen}}
\def\OKey{\mathsf{OKey}}
\def\OCor{\mathsf{OCor}}
\def\OSEnc{\mathsf{OSEnc}}
\def\OEnc{\mathsf{OEnc}}
\def\OChal{\mathsf{OChal}}
\def\OTGen{\mathsf{OTgen}}
\def\OTag{\mathsf{OTag}}
\def\OVerif{\mathsf{OVer}}
\def\anontrapcpa{\mathsf{trap\mhyf cpa}}
\def\wanontrapcpa{\mathsf{w\mhyf anon\mhyf trap\mhyf cpa}}
\def\anonctcpa{\mathsf{ct\mhyf cpa}}
\def\wanonctcpa{\mathsf{w\mhyf anon\mhyf ct\mhyf cpa}}

% changed for SnP submission
% \def\fullcpa{\mathsf{full\mhyf cpa}} 
% \def\anoncpa{\mathsf{anon\mhyf cpa}} 
% \def\anoncca{\mathsf{anon\mhyf cca}} 
% \def\trapcma{\mathsf{trap\mhyf cma}}
% \def\ctcma{\mathsf{ct\mhyf cma}}
% \def\mprcma{\mathsf{mpr\mhyf cma}}
% changed for SnP submission
\def\fullcpa{{full\mhyf cpa}} 
\def\anoncpa{{anon\mhyf cpa}} 
\def\anoncca{{anon\mhyf cca}} 
\def\trapcma{{trap\mhyf cma}}
\def\ctcma{{ct\mhyf cma}}

\def\Core{\mathsf{Core}}
\def\Finalize{\mathsf{Finalize}}

\mathchardef\mhyf="2D
\def\kMDDHo{\mathsf{k\mhyf MDDH}_1}
\def\kMDDHw{\mathsf{k\mhyf MDDH}_2}
\def\pmh{\mathsf{PMH}}

\def\Span{\mathsf{span}}
\def\Game{{\mathbf{Game}}}
\def\mcmn{m}

\def\ibe{\mathsf{IBE}}
\def\ibbe{\mathsf{IBBE}}
\def\ibr{\mathsf{IBR}}
\def\pfnc{\mathsf{R}}
\def\ipe{\mathsf{IPE}}
\def\zipe{\mathsf{ZIPE}}
\def\nipe{\mathsf{NIPE}}
\def\poipe{\mathsf{PO\mhyf IPE}}
\def\pozipe{\mathsf{PO\mhyf ZIPE}}
\def\ponipe{\mathsf{PO\mhyf NIPE}}
\def\pomvme{\mathsf{PO\mhyf MVME}}
\def\ipePrdf{\mathpzc{i}}
\def\zipePrdf{\mathpzc{z}}
\def\nipePrdf{\mathpzc{n}}
\def\mvmePrdf{\mathpzc{m}}
\def\po{\mathpzc{po}}
\def\mvme{\mathpzc{mvme}}

\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\def\proto{\mathsf{P}_1}
\def\prott{\mathsf{P}_2}

% \def\tR{\widetilde{\matx{R}}}
% \def\R{\matx{R}}
% \def\Rl{\matx{R}_\el}
% \def\Rr{\matx{R}_\ar}
% \def\T{\matx{T}}
% \def\Tl{\matx{T}_\el}
% \def\Tr{\matx{T}_\ar}

\def\oraclb{\mathcal{O}_\bee}
\def\oracls{\mathcal{O}^*}

\def\I{\mathbf{I}}
\def\Zro{\mathbb{O}}
\def\zro{\mathbf{0}}
\def\msg{m}
\def\Msg{\mathbf{m}}
\def\MSg{\mathcal{M}}
\def\Sgn{\mathsf{Sign}}
\def\PSgn{\mathsf{PSign}}
\def\ufxcma{\mathsf{Uf}\mhyf\mathsf{XCMA}}
\def\ufcma{\mathsf{Uf}\mhyf\mathsf{CMA}}
\def\rrlink{\mathsf{RR}\mhyf\mathsf{Link}}
\def\sign{\sigma}
\def\tsign{\widetilde{\sigma}}

\def\Sig{\Sigma}
\newcommand{\sig}[1][]{\sigma_{#1}}
\newcommand{\sigR}[1][]{\sigma'_{#1}}
\newcommand{\hsig}[1][]{\widehat{\sigma}_{#1}}
\newcommand{\tsig}[1][]{\widetilde{\sigma}_{#1}}
\newcommand{\tsigR}[1][]{\widetilde{\sigma}'_{#1}}

\newcommand{\xptb}{[b]}
\newcommand{\xpz}{{[0]}}
\newcommand{\xpo}{{[1]}}
\newcommand{\xpb}{{[\bee]}}
\newcommand{\xpd}{{[\dee]}}
\newcommand{\xpomb}{{[1-\bee]}}

\def\etal{\textit{et al.\ }}

\def\dforall{\overset{*}{\forall}}
\def\dontcare{\_}
\def\Fact{\mathsf{F}}

\newcommand{\arw}[1]{\underset{\substack{\uparrow \\ {\tau(j)^\text{th}}}}{#1}}
\def\UU{\mathcal{U}}

\newcommand{\bigO}[1]{\mathcal{O}(#1)}
\newcommand{\bigOm}[1]{\Omega(#1)}
\newcommand{\bigTh}[1]{\Theta(#1)}
\newcommand{\smallO}[1]{{o}(#1)}
\newcommand{\smallOm}[1]{\omega(#1)}



